MCLFIQ: Mobile Contactless Fingerprint Image Quality

We propose MCLFIQ: Mobile Contactless Fingerprint Image Quality, the first quality assessment algorithm for mobile contactless fingerprint samples. To this end, we re-trained the NIST Fingerprint Image Quality (NFIQ) 2 method, which was originally designed for contact-based fingerprints, with a synthetic contactless fingerprint database. We evaluate the predictive performance of the resulting MCLFIQ model in terms of Error-vs.-Discard Characteristic (EDC) curves on three real-world contactless fingerprint databases using three recognition algorithms. In experiments, the MCLFIQ method is compared against the original NFIQ 2.2 method, a sharpness-based quality assessment algorithm developed for contactless fingerprint images \rev{and the general purpose image quality assessment method BRISQUE. Furthermore, benchmarks on four contact-based fingerprint datasets are also conducted.} Obtained results show that the fine-tuning of NFIQ 2 on synthetic contactless fingerprints is a viable alternative to training on real databases. Moreover, the evaluation shows that our MCLFIQ method works more accurate and robust compared to all baseline methods on contactless fingerprints. We suggest considering the proposed MCLFIQ method as a \rev{starting point for the development of} a new standard algorithm for contactless fingerprint quality assessment.

==> Coverletter/data.tex <==
%% First author details
\def\authorname{Jannis Priesnitz}
\def\authrinstitution{Hochschule Darmstadt}
\def\authorstreet{Haardtring}
\def\authorstreetnumber{100}
\def\authorcity{Darmstadt}
\def\authorpostalcode{64295}
\def\authorcountry{Germany}

%% Co-author details
\def\coauthorslist{Axel~Weißenfeld, Christian~Rathgeb, Berhard~Strobl, Ralph~Lessmann, and Christoph~Busch}

%% Logos
\def\logobottomleft{figures/logos/dasec}
\def\logobottomcenter{figures/logos/athene_en}
\def\logobottomright{figures/logos/hda}

%% Article details
\def\articletitle{MCLFIQ: Mobile Contactless Fingerprint Image Quality}
\def\articleid{TBIOM-2023-06-0057}
\def\articlejournalabbreviation{IEEE TBIOM}
\def\articlejournal{IEEE Transactions on Biometrics, Identity and Behavior }
\def\articleinterest{
it presents a novel quality assessment algorithm for contactless finger images acquired in mobile scenarios.  
First, if defines framework conditions for pre-processing contactless fingerprint images in order to achieve sample consistency and to make all images suitable for quality assessment using our method.
A random forest is  then re-trained using a synthetically generated contactless fingerprint database. Finally, the newly generated model, referred to as MCLFIQ is tested using three real world contactless fingerprint databases. For the evaluation, we consider two recognition workflows, one commercial-off-the-shelf system and one which is based on open-source algorithms. Our MCLFIQ model is benchmarked against the latest version of NFIQ 2 (NFIQ 2.2) and a quality metric, which is based on sharpness and was developed for contactless fingerprint images in terms of Error vs. Discard Characteristic (EDC) curves.

Our results show  significant improvement of prediction accuracy compared to both baseline algorithms. 
\end{itemize}

}
\def\articlecontribution{propose a new quality assessment algorithm for contactless fingerprints and test it using real world databases and recognition workflows. 
}

%% Cover letter details
\def\letterdate{\today}

%% Revision cover letter
\def\articledecison{major revision} % minor revision or major revision
\def\articlenumreviewers{3}

%% Response letter
\def\revisionnumber{r1}
\def\reviewsdir{reviews/}

%% Change only if needed
\def\authoraddress{
\authrinstitution{} \\
\authorstreet{} \authorstreetnumber{} \\
\authorpostalcode{}, \authorcity{} \\
\authorcountry{}
}
\providecommand\authorsignature{}
\renewcommand{\authorsignature}{
\vspace{-1mm}
%\includegraphics[height=1cm]{figures/signature}
}

\providecommand\logos{}
\renewcommand{\logos}{ % choose logos as appropriate
\includegraphics[height=0.75cm]{\logobottomleft} \hfill
\includegraphics[height=0.75cm]{\logobottomcenter} \hfill
\includegraphics[height=0.75cm]{\logobottomright}
}

\def\letterrecipient{Editor}
\def\letteropening{Dear Sir or Madam,}
\def\letterclosing{Sincerely,}

\def\responseletterheading{
\begin{center}
\LARGE\textbf{Response Letter} \par \smallskip
\large\textbf{\articletitle{}} \par
\end{center}
}

\providecommand\reviewheading{}
\renewcommand{\reviewheading}[1]{
\section*{#1}
}

\providecommand\reviewcomment{}
\renewcommand{\reviewcomment}[3]{
\textbf{\textcolor{#3}{#1}} \par \smallskip
#2 \par \medskip
}

\def\EASY{OliveGreen}
\def\MEDIUM{Orange}
\def\HARD{Red}
\def\DONE{Black}


==> Coverletter/reviews/editor.tex <==
\reviewheading{Editor}

\reviewcomment{
I am sure that the provided suggestions will be useful to improve your manuscript.
Be advised that a possible final acceptance is strictly constrained by the full reviewers' satisfaction with your revisions. In addition, correct language is of paramount importance to publish in a high-ranked journal. Please thoroughly review the text.
Therefore, I invite you to submit a new version of the manuscript with detailed responses to reviewers.
}
{
We can confirm that we conducted a in-depth revision of the manuscript. We conducted in total 67 new experiments in order to adress the reviewer comments. Furthermore, we revised the entire manuscript regarding written text accuracy and language mistakes. Please note that we did only highlight major changes in \textcolor{blue}{blue}.
}
{\DONE}

%\reviewcomment{
%COMMENT 0.2
%}
%{
%COMMENT RESPONSE
%}
%{\EASY}
%
%\reviewcomment{
%COMMENT 0.3
%}
%{
%COMMENT RESPONSE
%}
%{\MEDIUM}
%
%\reviewcomment{
%COMMENT 0.4
%}
%{
%COMMENT RESPONSE
%}
%{\HARD}


==> Coverletter/reviews/reviewer1.tex <==
\reviewheading{Review 1}

\reviewcomment{
In this paper, the authors specialized the well-known NFIQ 2 algorithm for fingerprint quality assessment of images coming from mobile devices. They called, accordingly, mobile contactless fingerprint image quality algorithm (MCLFIQ algorithm). This paper is the follow-up of previous work by the same authors:
(...)
Thus the only novelty is to re-train the NFIQ 2 random forest by using synthetic images and testing on real fingerprint images. It is also worth noting that the authors are part of the research group implementing NFIQ 2.
}
{
The authors share the opinion that research should be well-founded and justified. For this reason we re-use databases and algorithms proposed so far. Nevertheless, the reviewer is partly correct with his statement that this paper is a follow-up of "Touchless fingerprint sample quality: Prerequisites for the applicability of nfiq 2.0". Our 2020 paper acts as problem statement and motivation for this paper. However this work goes far beyond our previous one. 
}
{\DONE}

\reviewcomment{
First, Table IV shows the most relevant features adopted by MCLFIQ and the original NFIQ after training (it is not clearly indicated). Very interesting map; however, the authors spent a few words commenting on the RF ensemble’s choice. They wrote:
“In particular, the two features ROI Relative Orientation Map Coherence Sum and Orientation Certainty Level Mean alone share over 50\% of the whole feature importance. Both features are mainly based on sharpness measures, which is seen as the most crucial point for contactless fingerprint sample quality assessment.”
To strengthen the impact of this “importance map” (BTW, no formal definition of “importance” is given over the paper), in my opinion, the authors should have better connected these numbers with a more formal definition of “utility,” “fidelity,” and “character.” These terms are only introduced (p. 3). However, they are no longer used: thus, it is not clear if they are mere high-level terms or measures that can be assessed somehow. The unique exception is “utility,” thanks to the definition being closer to a real measurement than the others. Due to this poor connection with ISO definitions, the remainder comments appear not theoretically or experimentally supported, and their impact is reduced from a scientific viewpoint.
}
{
We thank the reviewer for the suggestion. We revised this section and provided a definition of feature importance which aligns to the ISO standards and further discuss the table regarding the terms "utility", "fidelity", and "character" which should be beneficial to understand the results better. It should be noted that ISO/IEC 29794-1 does not provide a more formal definition than the one included in our work.
}
{\DONE}

\reviewcomment{
The other parts of the paper show that the MCLFIQ is in line with the state-of-the-art, with some exceptions in Fig. 9. Of course, it is worth remarking that all explored data sets exhibit a small user population. Thus, the results should be contextualized on that user population size. This is not a big problem because the scenario is focused on mobile devices, where many hands are not expected to use them. On the contrary, in this scenario is much more interesting to assess the algorithm performance on different devices. This is not the case in the reported experimental results. The non-mobile contactless fingerprint scenario case would be different because we have similar constraints to the contact fingerprint one.
}
{
Unfortunately to the authors' knowledge there are no larger databases freely available which fit to the requirements of our experiments. We added a statement on the sizes of the considered databases and its possible impact on the conducted experiments.
}
{\DONE}

\reviewcomment{
To conclude the review, the absence of the following "ad excludendum" experiment set is disappointing: the authors claim that MCLFIQ is suitable for contactless fingerprint image quality, but how about the contact-based one? They showed that NFIQ 2 is also suitable in contactless-based scenarios. Thus, I would expect a reversed experiment to show that MCLFIQ matches this one much better than the contact-based one. Otherwise, it is just a n+1 quality assessment method, without the peculiarity claimed by the authors. It can be a candidate as an ISO reference only because it is an incremental modification of another ISO reference, namely, the NFIQ 2 method.
}
{
We appreciate the reviewers suggestion to do a counter-experiment on contact-based databases. We also benchmarked 5 contact-based fingerprint databases. The results showcase that both models perform best for their respective use-case.  

}
{\DONE}


==> Coverletter/reviews/reviewer2.tex <==
\reviewheading{Review 2}

\reviewcomment{
In this paper, the authors propose a quality evaluation tool for contactless fingerprint images by re-training the random forest in NFIQ2, which is a quality evaluation tool for fingerprint images acquired by contact-type sensors, with fingerprint images acquired by contactless sensors. Although the effort to study the image quality evaluation of fingerprint images targeting contactless fingerprint recognition can be positively recognized, the novelty is extremely limited because it only re-trains the random forest part in NFIQ2. The training data created for re-training are fingerprint images synthesized by SynCoLFinGer and labeled with quality labels according to SynCoLFinGer. Therefore, the performance of the proposed method depends on that of SynCoLFinGer. Therefore, this paper is considered to be a case study rather than a proposal of a new method.
}
{
The authors appreciate that the reviewer recognizes the effort we put into this work. However, we do not share the opinion that the novelty of out proposal is extremely limited taking the following aspects into account: 
\begin{itemize}
    \item Our related work study shows that so far no proposal of a mobile contactless fingerprint quality assessment method including a broader and comparative evaluation has been conducted yet.
    \item The random forest model drastically changed for MCLFIQ re-training (c.f. Table 4 in the paper)
    \item To the authors knowledge no annotated contactless fingerprint database exists for re-training the classifier. 
\end{itemize}
Nevertheless the reviewer is correct that the performance depends on the used synthetic data and with his suspicion that real data might perform different. We added a statement on that in the manuscript. 
}
{\DONE}

\reviewcomment{
For example, instead of the NFIQ2 framework, image feature extraction such as Convolutional Neural Networks (CNNs) can be used for quality evaluation. If the performance of the NFIQ2 framework is superior to that of the CNN or its derivatives, the effectiveness of the method is acceptable to the reader. Although CNNs are not necessarily better in this case because they are also highly dependent on training data, the effectiveness of methods such as CNNs in biometrics has been demonstrated, so a comparison with CNNs is strongly required.
}
{
The suggestion of the reviewer is in general reasonable. However, CNN-based methods have distinct drawbacks: 
\begin{itemize}
    \item No easy way to provide actionable feedback to user or operator: With our proposal it is possible to make well-founded decision based one scores of individual quality components. 
    \item CNNs tend to generalize poor to new data: The goal of this proposal is to suggest a starting point for a new standard algorithm. The authors suspect that a well-generalizing CNN-based methods can be trained with the available databases. 
    \item CNNs pose a huge challenge when it comes to explanation. Their intricate architectures and numerous parameters can make it hard to decipher the underlying decision-making processes. In contrast,  machine learning methods based on hand-crafted features offer a more transparent and interpretable approach, which makes it easier to understand and communicate the reasoning behind their predictions. This interpretability advantage provides valuable insights and fosters trust in the models' results.
\end{itemize}
For this reason the authors have concerns that CNNs are a well-suited alternative to out proposed method. Nevertheless, the reviewer is correct with his objection, that CNN-based methods should also be investigated. Given the amount of time and the page limit we could not include such a metric in this manuscript. However, we added a statement on this in the manuscript and will further research this topic. 

As a compromise we added experiments using the well-established NR-IQA algorithm BRISQUE. We re-trained the algorithm using the the same database like for MCLFIQ but used color images since they work better with BRISQUE. It turned out that the results are inferior in most cases which could also be an indication for CNN-based methods. 
}
{\DONE}

\reviewcomment{
The major difference between MCLFIQ and NFIQ2 is whether random forests are trained on contact or contactless fingerprint images. In the tests, the authors evaluated the performance of MCLFIQ and NFIQ2 using contactless fingerprint images, so the higher performance of MCLFIQ is to be expected. The authors should also experiment with the use of contact fingerprint images in the tests, although this would confirm the importance of consistency between the training data and its purpose as a tool.
Table IV summarizes the important features of MCLFIQ and NFIQ2, respectively. As mentioned above, the results confirm the trend of differences between contact and contactless fingerprint images in the training data. Since the trend should be different when contact fingerprint images are used in the test, it is possible to check the differences between contact and contactless fingerprint images comprehensively.
}
{
We appreciate the reviewers suggestion to do a counter-experiment on contact-based databases. We also benchmarked 5 contact-based fingerprint databases. The results showcase that both models perform best for their respective use-case.  
}
{\DONE}

\reviewcomment{
In this paper, NFIQ2, NFIQ2.0, NFIQ2.1, and NFIQ2.2 are used. A detailed description of the differences between these versions is required. It is also unclear whether the authors use these versions differently.
}
{
We clearified this issue. 
}
{\DONE}


==> Coverletter/reviews/reviewer3.tex <==
\reviewheading{Reviewer 3}

\reviewcomment{
This paper presents a quality assessment method designed for touchless fingerprint images acquired using mobile devices. Specifically, NFIQ 2 has been re-trained by using synthetic touchless images. The paper presents promising results and interesting observations. However, there are some major concerns to be addressed to make the paper publishable.}
{
We appreciate the reviewers opinion that our work presents promising results and interesting observations. 
}
{\DONE}

\reviewcomment{
- The paper states “We suggest to further investigate on contactless fingerprint quality assessment and consider the proposed MCLFIQ approach as a candidate for a new standard algorithm”. I think that this work could be a good starting point for new standards. However, in its current form, its accuracy is strictly related to preprocessing techniques, which can be different according to the acquisition setup and environmental conditions. I suggest modifying this period.
}
{
The reviewer is correct with his observation that this statement was presumptuous. We mitigated our statement. 
}
{\DONE}

\reviewcomment{
- The paper does not consider a relevant problem of touchless fingerprint recognition systems based on mobile devices, which consists of finger placement. Finger images acquired with different angles in the three-dimensional space can present perspective distortions and show different portions of the ridge pattern. I think that this aspect is particularly relevant for a quality assessment method designed for touchless fingerprint images acquired using mobile devices. Therefore, this aspect should be properly discussed in the text.
}
{
We thank the reviewer for this valuable statement. We added a discussion on this in the manuscript. 
}
{\DONE}

\reviewcomment{
- Since the proposed method requires a preprocessing step, a detailed description of the implemented methods should be provided in the text.}
{
We also present more details on the pre-processing pipeline. However taking the page-limit into account we had to be concise with this. It should be noted that the used pre-processing is not a key-contribution of the work and the used pipeline can be studied in the cited literature. 
}
{\DONE}

\reviewcomment{
- Since many existing fingerprint recognition systems only evaluate minutiae features, I suggest using an additional matcher for evaluating the performance of the proposed method. Specifically, I suggest using the open-source implementation of the NIST fingerprint matcher, which is a well-known algorithm based only on minutiae features.}
{
We are happy to announce that we also conducted all experiments using the NBIS workflow which further supports our findings.  
}
{\DONE}


\reviewcomment{
- It is not clear if the proposed method can be applied in live applications to simplify the acquisition process. I suggest evaluating the required computational time, to estimate the maximum number of supported frames per second in real-time applications.
}
{
So far we did not yet include the method into a mobile application. For this reason, we also did not report any time measurements. We conducted measurements on a notebook computer and it turned out that MCLFIQ is slightly faster than NFIQ 2.2. Due to the limited page size we did not include this into the manuscript but we are happy to provide timing measurements as supplemental material.  
}
{\DONE}

\reviewcomment{
- The paper should be proofread for English errors.}
{
We revised the entire manuscript for English errors. 
}
{\DONE}
